Exploiting Energy Accumulation Against Co-channel Interference in Wireless Energy Harvesting MIMO Relaying

This paper investigates a three-node multiple-input multiple-output relay system suffering from co-channel interference (CCI) at the multi-antenna relay. Contrary to the conventional relay networks, we consider the scenario that the relay is an energy harvesting (EH) node and has no embedded energy supply. But it is equipped with a rechargeable battery such that it can harvest and accumulate the harvested energy from RF signals sent by the source and co-channel interferers to support its operation. Leveraging the inherent feature of the considered system, we develop a novel accumulate-then-forward (ATF) protocol to eliminate the harmful effect of CCI. In the proposed ATF scheme, at the beginning of each transmission block, the relay can choose either EH operation to harvest energy from source and CCI or information decoding (ID) operation to decode and forward source's information while suffering from CCI. Specifically, ID operation is activated only when the accumulated energy at the relay can support an outage-free transmission in the second hop. Otherwise, EH operation is invoked at the relay to harvest and accumulate energy. By modeling the finite-capacity battery of relay as a finite-state Markov Chain (MC), we derive a closed-form expression for the system throughput of the proposed ATF scheme over mixed Nakagami-m and Rayleigh fading channels. Numerical results validate our theoretical analysis, and show that the proposed ATF scheme with energy accumulation significantly outperforms the existing one without energy accumulation.

==> Markov_relay.tex <==
\section{Markov Model of Relay battery}

The proposed ATF protocol described in the previous section will lead to a specific charging and discharging behaviors of relay battery. To analyze the performance of the considered network with the ATF protocol, we first need to model this dynamic behaviors of the relay battery. To this end, we adopt a finite-state Markov chain (MC) to model the relay battery behaviors and find the corresponding stationary distribution of the formulated MC. %This is in contrast to the continuous storage model adopted in \cite{Nasir_Tcom_2015_Wire}.

\subsection{Battery model and Energy Discretization}
In this paper, we consider that the relay is equipped with a finite-capacity battery. To characterize the state of the battery, we follow \cite{Krikidis_CL_2012_RF} and adopt a discrete-level battery model. More specifically, We use $C$ to denote the capacity of the relay battery and $Q$ to denote the number of discrete energy levels excluding the empty level. Then, the $i$th energy level of the relay battery can be expressed as ${\varepsilon_i} = iC/Q$, $i  \in \left\{  0,1,2 \cdots Q\right\}$. We define state ${S_i}$ as the relay residual energy in the battery being ${\varepsilon_i}$. The transition probability $T_{i,j}$ is defined as the probability of the transition from state $S_i$ to state $S_j$. With the adopted discrete-level battery model, the amount of harvested energy can only be one of the discrete energy level of the battery. The discretized amount of harvested energy in Mode I or II is thus defined as
\begin{equation}\label{eq:discrete_EI}
{E_{\rm I}} \buildrel \Delta \over = {\varepsilon _{j}}, \quad {j} = \arg \mathop {\max }\limits_{i \in \left\{ {0,1, \cdots ,Q} \right\}} \bigg\{{\varepsilon _i}:{\varepsilon _i} <  {\tilde E_{\rm I}}\bigg\},
\end{equation}
\begin{equation}\label{}
{ E_{\rm II}} \buildrel \Delta \over = {\varepsilon _{j}}, \quad {j} = \arg \mathop {\max }\limits_{i \in \left\{ {0,1, \cdots ,Q} \right\}} \bigg\{{\varepsilon _i}:{\varepsilon _i} <  {\tilde E_{\rm II}}\bigg\},
\end{equation}

On the other hand, when $D$ adopts the $\rm X$, $\rm X \in \left\{{\rm MRC, ZF, MMSE}\right\}$,  combining scheme, the discretized value of the required outage-free energy at the relay in Mode III should be defined as
\begin{equation}\label{}
{E_R^{\rm X}} \buildrel \Delta \over =
\left\{
\begin{matrix}
\begin{split}
&{\varepsilon _{j}}, \quad \text{if} \quad {{P_R^{\rm X}} \over 2} \le C \\
& \infty, \quad \text{if} \quad {{P_R^{\rm X}} \over 2} > C
\end{split}
\end{matrix}
\right.,
\end{equation}
where $j= \arg \mathop {\min }\limits_{i \in \left\{ {0,1, \cdots ,Q} \right\}} \bigg\{{\varepsilon _i}:{\varepsilon _i} \ge {{P_R^{\rm X}}/2}\bigg\}$, and $P_R^{\rm X}$ is defined in (\ref{eq:relay_power_threecase}). Note that the factor $\frac{1}{2}$ is introduced because the relay performs information forwarding only during the second time slot.

\subsection{Markov Chain of Relay Battery}
We are now ready to describe the relay behaviors in the proposed ATF scheme mathematically. Let $\Upsilon \left[ {n} \right] \in \left\{ {{\Upsilon _{\rm {I}}},{\Upsilon _{\rm {II}}},{\Upsilon _{\rm {III}}}} \right\}$, $n \in \left\{ {1,2,3 \cdots } \right\}$, denote the operation mode of the relay during the $n$th transmission block, where ${\Upsilon _{\rm {I}}}$, ${\Upsilon _{\rm {II}}}$ and ${\Upsilon _{\rm {III}}}$ represent Mode I, II and III, respectively. We denote by ${\Delta }[n]$ the residual energy accumulated by the relay at the beginning of the $n$th transmission block. Recall that in Sec. II, we define $\lambda \left[{n}\right]$ as the accumulated energy status and $\kappa \left[{n}\right]$ to be the ID indicator of the relay. According to the principle of the proposed scheme, when the $\rm X$, $\rm X \in \left\{{\rm MRC, ZF, MMSE}\right\}$, combining technique is implemented at $D$, we then readily have the following equations
\begin{equation}\label{eq:protocol_in_math_1}
\lambda \left[ n \right] = \left\{ {
\begin{matrix}
\begin{split}
   &0,\quad \text{if} \quad  {\Delta}[n] <  {E_R^{\rm X}} \\
   &1,\quad \text{if} \quad   {\Delta}[n] \ge  {E_R^{\rm X}} \\
\end{split}
\end{matrix}
  } \right.,
\end{equation}

\begin{equation}\label{}
\Upsilon \left[ n \right] = \left\{ {
\begin{matrix}
\begin{split}
   &{\Upsilon _{\rm {I}}},\quad \text{if} \quad  \left\{\lambda \left[ n \right] = 0\right\},  \\
   &{\Upsilon _{\rm {II}}},\quad \text{if} \quad   \left\{\lambda \left[ n \right] = 1 \right\} \cap \left\{\kappa \left[{n}\right] =0 \right\},  \\
   &{\Upsilon _{\rm {III}}},\quad \text{if} \quad   \left\{\lambda \left[ n \right] = 1 \right\} \cap \left\{\kappa \left[{n}\right] =1 \right\}.  \\
\end{split}
\end{matrix}
  } \right.
\end{equation}

\begin{equation}\label{eq:protocol_in_math_3}
{\Delta}[n+1] = \left\{ {
\begin{matrix}
\begin{split}
   &{\min \bigg \{{\Delta}[n] + {E_{\rm I}}, C \bigg\}, \quad \text{if} \quad \Upsilon \left[ n \right] = {\Upsilon _{\rm {I}}}}  ,\\
   &{\min \bigg \{{\Delta}[n] + {E_{\rm II}}, C \bigg\}, \quad \text{if} \quad \Upsilon \left[ n \right] = {\Upsilon _{\rm {II}}}} ,\\
   &{{\Delta}[n]-{E_R^{\rm X}}, \quad \text{if} \quad \Upsilon \left[ n \right] = {\Upsilon _{\rm {III}}}}. \\
\end{split}
\end{matrix}
  } \right.
\end{equation}

With the mathematical description of the proposed ATF scheme and the MC model defined above, we are now ready to evaluate the state transition probabilities of the MC of relay battery. Inspired by \cite{Krikidis_CL_2012_RF}, we can summarize all transition probabilities into the following eight general cases.
\subsubsection{The battery remains empty (${S_0}\quad to\quad {S_0}$)}
Mode I is activated when the relay has an empty battery. Furthermore, the transition ends with an empty battery, which indicates that the discretized amount of harvested energy ${E_{\rm I}}$ during this block must be zero. From the definition of discretization given in (\ref{eq:discrete_EI}), condition $\tilde E_{\rm I}< {\varepsilon _1} = C/Q$ must hold such that the continuous harvested energy can be discretized to zero. The transition probability of this case can thus be expressed as
\begin{equation}
\begin{split}
{T_{0,0}}& = \Pr \bigg\{ \Upsilon \left[ n \right]  =  {\Upsilon _{\rm {I}}}, {E_{\rm I}}=0 \left| {{\Delta}[n]=0} \right. \bigg\}\\
&= \Pr \bigg\{ {\tilde E_{\rm I}}<C/Q \bigg\}\\
&= {F_{\tilde E_{\rm I}}}\left( C/Q \right),\\
\end{split}
\end{equation}
where ${F_{\tilde E_{\rm I}}}\left( x \right)$ is the CDF of the harvested energy in Mode I given in (\ref{eq:CDF_EI}).


\subsubsection{The battery is fully charged (${S_0}\quad to\quad {S_Q}$)}In this transition case, Mode I is performed to charge the battery from empty to full. The amount of the harvested energy $\tilde E_{\rm I}$ during this operation should be greater than the battery capacity $C$. Thus the transition probability can be characterized as
\begin{equation}
\begin{split}
{T_{0,Q}} & = \Pr \bigg\{ \Upsilon \left[ n \right]  =  {\Upsilon _{\rm {I}}}, {E_{\rm I}} = C \left| {{\Delta}[n]=0} \right. \bigg\}\\
& =1-{F_{\tilde E_{\rm I}}}\left( C \right).
\end{split}
\end{equation}

\subsubsection{The battery is partially charged (${S_0}\quad to\quad {S_i}$ with $0 < i < Q$)}
Similar as the previous case, the transition probability can be calculated as
\begin{equation}
\begin{split}
T_{0,i} & =\Pr \bigg\{ \Upsilon \left[ n \right]  =  {\Upsilon _{\rm {I}}}, {E_{\rm I}} = iC/Q \left| {{\Delta}[n]=0} \right. \bigg\}\\
& = \Pr \left\{ iC/Q < \tilde E_{\rm I} <  (i+1)C/Q \right\}\\
&={F_{\tilde E_{\rm I}}}\left( (i+1)C \over Q \right) - {F_{\tilde E_{\rm I}}}\left( iC \over Q \right).
\end{split}
\end{equation}

\subsubsection{The non-empty and non-full battery remains unchanged (${S_i}\quad to\quad {S_i}$ with $0 < i  < Q$)}\label{an1}
We can deduce that this transition case happens when Mode I or Mode II is operated and the corresponding harvested energy is zero (i.e. ${E_{\rm I}}=0$ or ${E_{\rm II}}=0$). From the mathematical description given in (\ref{eq:protocol_in_math_1})-(\ref{eq:protocol_in_math_3}), the probability of the current transition can be expressed as
\begin{equation}\label{eq:T_ii}
\begin{split}
{T_{u}^{i,i}}  = & \Pr \bigg\{ \left\{ \Upsilon \left[ n \right]  =  {\Upsilon _{\rm {I}}}, {E_{\rm I}}=0 \left| {{\Delta}[n]=\varepsilon _i } \right. \right\} \cup\\
& \left\{  \Upsilon \left[ n \right]  =  {\Upsilon _{\rm {II}}}, {E_{\rm II}}=0 \left| {{\Delta}[n]=\varepsilon _i} \right.  \right\} \bigg\} \\
 = &\Pr \left\{ {E_R^{\rm X}} > \varepsilon _i \right\}\Pr \left\{ {E_{\rm I}}=0 \right\}+\\
&\Pr \left\{ {E_R^{\rm X}} \le \varepsilon _i \right\} \Pr \left\{ \kappa \left[{n}\right] =0 \right\} \Pr \left\{ {E_{\rm II}}=0 \right\}\\
=& \Pr \left\{   {{P_R^{\rm X}} \over 2} > iC/Q \right\} \Pr \left\{   {\tilde E_{\rm I}} <C/Q \right\}+\\
&\Pr \left\{   {{P_R^{\rm X}} \over 2} \le iC/Q \right\} \Pr \left\{ \kappa \left[{n}\right] =0 \right\} \Pr \left\{ {\tilde E_{\rm II}}<C/Q\right\}\\
= &\left[1-{F_{\rm X}}\left( 2iC \over Q \right)\right]{F_{\tilde E_{\rm I}}}\left( C \over Q \right)+\\
& \left[{F_{\rm X}}\left( 2iC \over Q \right)\right]{{ F}_{\tilde E_{\rm II}}}\left( C \over Q \right)\Pr \left\{ \kappa \left[{n}\right] =0 \right\},
\end{split}
\end{equation}
where ${{ F}_{\tilde E_{\rm II}}}\left( x\right)$ is the CDF of the harvested energy in Mode II and ${F_{\rm X}}\left(\cdot\right)$ can be equal to (\ref{eq:CDF_MRC}), (\ref{eq:CDF_ZF}) or (\ref{eq:CDF_MMSE}) depending on the adopted linear combining scheme at destination. The only unknown term in (\ref{eq:T_ii}) is $\Pr \left\{ \kappa \left[{n}\right] =0 \right\}$, which denotes the probability that the relay suffers from outage when it tries to decode the source's information. To derive this, we have
\begin{equation}\label{eq:pr_kappa}
\begin{split}
 \Pr \left\{ {\kappa \left[ n \right] = 0} \right\} &= \Pr \left\{ {{\gamma _R} < \mu } \right\} \\
 & = \Pr \left\{ {\frac{{{P_0}{{\left\| {{{\bf{h}}_0}} \right\|}^2}}}{{Y + \sigma _R^2}} < \mu } \right\} \\
 & = 1 - \int_0^\infty  {\int_{y + \sigma _R^2}^\infty {{f_Z}\left( z \right)dz} } {f_Y}\left( y \right)dy,
\end{split}
\end{equation}
where $Z = {P_0}{\left\| {{{\bf{h}}_0}} \right\|^2}/\mu $ follows a gamma distribution with shape parameter $m_sN_s$ and average power $N_s {P_0} \Omega_0/\mu$. Moreover, the PDF of $Y$ has been presented in (\ref{eq:PDF_Y}). With this, we can obtain a closed-form expression for the above double integral given by (\ref{eq:kappa_expression}) on top of next page. By inserting (\ref{eq:kappa_expression}) into (\ref{eq:T_ii}), we can obtain the transition probability ${T_{u}^{i,i}}$.


\begin{figure*}[!t]
% ensure that we have normalsize text
%\normalsize
%% Store the current equation number.
%\setcounter{mytempeqncnt}{\value{equation}}
%% Set the equation number to one less than the one
%% desired for the first equation here.
%% The value here will have to changed if equations
%% are added or removed prior to the place these
%% equations are referenced in the main text.
%\setcounter{equation}{30}.
\begin{equation}\label{eq:kappa_expression}
\begin{split}
 \Pr \left\{ \kappa \left[{n}\right] =0 \right\} = 1 - \exp \left( { - {{{m_s}{\sigma_R ^2}\mu } \over {{P_0}{\Omega _0}}}} \right)\sum\limits_{i = 1}^{{N_s}} {\sum\limits_{j = 1}^{{m_c}} {\sum\limits_{k = 0}^{{m_s}{N_s} - 1} {{{{A_{i,j}}{{\left( {{{{m_s}\mu } \over {{P_0}{\Omega _0}}}} \right)}^k}} \over {\Gamma \left( j \right)k!}}} } }  \sum\limits_{l = 0}^k {{{{{\binom{k}{l}\left( {{\sigma_R ^2}} \right)}^{k - l}}\left( {j - 1 + l} \right)!} \over {{{\left( {{{{m_c}} \over {{P_l}{\Omega _l}}} + {{{m_s}\mu } \over {{P_0}{\Omega _0}}}} \right)}^{j + l}}}}} .
\end{split}
\end{equation}
% Restore the current equation number.
%\setcounter{equation}{\value{mytempeqncnt}}
% IEEE uses as a separator
\hrulefill
% The spacer can be tweaked to stop underfull vboxes.
\vspace*{4pt}
\end{figure*}

%\newcounter{mytempeqncnt3}
%\begin{figure*}[!t]
% ensure that we have normalsize text
%\normalsize
% Store the current equation number.
%\setcounter{mytempeqncnt}{\value{equation}}
% Set the equation number to one less than the one
% desired for the first equation here.
% The value here will have to changed if equations
% are added or removed prior to the place these
% equations are referenced in the main text.
%\setcounter{equation}{40}
%\begin{equation}
%\begin{split}
%{T_{u}^{i,i}}  &=  \Pr \bigg\{ \left\{ \Upsilon \left[ n \right]  =  {\Upsilon _{\rm {I}}}, {E_{\rm I}}=0 \left| {{\Delta}[n]=\varepsilon _i } \right. \right\} \cup \left\{  \Upsilon \left[ n \right]  =  {\Upsilon _{\rm {II}}}, {E_{\rm II}}=0 \left| {{\Delta}[n]=\varepsilon _i} \right.  \right\} \bigg\} \\
%& = \Pr \left\{ {E_R^{\rm X}} > \varepsilon _i \right\}\Pr \left\{ {E_{\rm I}}=0 \right\}+\Pr \left\{ {E_R^{\rm X}} \le \varepsilon _i \right\} \Pr \left\{ \kappa \left[{n}\right] =0 \right\} \Pr \left\{ {E_{\rm II}}=0 \right\}\\
%& = \Pr \left\{   {{P_R^{\rm X}} \over 2} > iC/Q \right\} \Pr \left\{   {\tilde E_{\rm I}} <C/Q \right\}+\Pr \left\{   {{P_R^{\rm X}} \over 2} \le iC/Q \right\} \Pr \left\{ \kappa \left[{n}\right] =0 \right\} \Pr \left\{ {\tilde E_{\rm II}}<C/Q\right\}\\
%& = \left[1-{F_{\rm X}}\left( 2iC \over Q \right)\right]{F_{\tilde E_{\rm I}}}\left( C \over Q \right)+\varphi \left[{F_{\rm X}}\left( 2iC \over Q \right)\right]{{ F}_{\tilde E_{\rm II}}}\left( C \over Q \right)
%\end{split}
%\end{equation}
% Restore the current equation number.
%\setcounter{equation}{\value{mytempeqncnt}}
% IEEE uses as a separator
%\hrulefill
%% The spacer can be tweaked to stop underfull vboxes.
%\vspace*{4pt}
%\end{figure*}

\subsubsection{The non-empty battery is partially charged (${S_i}\quad to\quad {S_j}$ with $0 < i < j< Q$)}In this transition, Mode I or Mode II operation should be operated with the residual energy being level $i$. Moreover, the discretized amount of energy harvested during Mode I or Mode II should be exactly equal to ${\varepsilon _{j - i}} = \left( {j - i} \right)C/L$. Similar to the previous case, the transition probability can be derived and expressed as (\ref{eq:Tij}) on top of next page.
%\newcounter{mytempeqncnt4}
\begin{figure*}[!t]
% ensure that we have normalsize text
%\normalsize
% Store the current equation number.
%\setcounter{mytempeqncnt}{\value{equation}}
% Set the equation number to one less than the one
% desired for the first equation here.
% The value here will have to changed if equations
% are added or removed prior to the place these
% equations are referenced in the main text.
%\setcounter{equation}{}
\begin{equation}\label{eq:Tij}
\begin{split}
{T_{i,j}}= &\Pr \bigg\{ \left\{ \Upsilon \left[ n \right]  =  {\Upsilon _{\rm {I}}}, {E_{\rm I}}={\varepsilon _{j - i}} \left| {{\Delta}[n]=\varepsilon _i } \right. \right\} \cup \left\{  \Upsilon \left[ n \right]  =  {\Upsilon _{\rm {II}}}, {E_{\rm II}}={\varepsilon _{j - i}} \left| {{\Delta}[n]=\varepsilon _i} \right.  \right\} \bigg\} \\
=&\left[1-{F_{\rm X}}\left( 2iC \over Q \right)\right]\left[{F_{\tilde E_{\rm I}}}\left( (j-i+1)C \over Q \right)- {F_{\tilde E_{\rm I}}}\left( (j-i)C \over Q \right)\right] +\\
 &\Pr \left\{ \kappa \left[{n}\right] =0 \right\} {F_{\rm X}}\left( 2iC \over Q \right)\left[{{ F}_{\tilde E_{\rm II}}}\left( (j-i+1)C \over Q \right)-{{ F}_{\tilde E_{\rm II}}}\left( (j-i)C \over Q \right)\right].
\end{split}
\end{equation}
% Restore the current equation number.
%\setcounter{equation}{\value{mytempeqncnt}}
% IEEE uses as a separator
\hrulefill
% The spacer can be tweaked to stop underfull vboxes.
\vspace*{4pt}
\end{figure*}

\subsubsection{The non-empty and non-full battery is fully charged (${S_i}\quad to\quad {S_Q}$ with $0 < i < Q$)}Similar as the previous case, we can express the transition probability of this case as (\ref{eq:TiQ}) on top of next page.
\newcounter{mytempeqncnt5}
\begin{figure*}[!t]
% ensure that we have normalsize text
%\normalsize
% Store the current equation number.
%\setcounter{mytempeqncnt}{\value{equation}}
% Set the equation number to one less than the one
% desired for the first equation here.
% The value here will have to changed if equations
% are added or removed prior to the place these
% equations are referenced in the main text.
%\setcounter{equation}{42}
\begin{equation}\label{eq:TiQ}
\begin{split}
{T_{i,Q}}
&=\Pr \bigg\{ \left\{ \Upsilon \left[ n \right]  =  {\Upsilon _{\rm {I}}}, {E_{\rm I}} \ge \varepsilon _{Q-i} \left| {{\Delta}[n]=\varepsilon _i } \right. \right\} \cup \left\{  \Upsilon \left[ n \right]  =  {\Upsilon _{\rm {II}}}, {E_{\rm II}} \ge \varepsilon _{Q-i} \left| {{\Delta}[n]=\varepsilon _i} \right.  \right\} \bigg\} \\
&=\left[1-{F_{\rm X}}\left( 2iC \over Q \right)\right]\left[1- {F_{\tilde E_{\rm I}}}\left( (Q-i)C \over Q \right)\right] + \Pr \left\{ \kappa \left[{n}\right] =0 \right\} \left[{F_{\rm X}}\left( 2iC \over Q \right)\right]\left[1-{{ F}_{\tilde E_{\rm II}}}\left( (Q-i)C \over Q  \right)\right].
\end{split}
\end{equation}
% Restore the current equation number.
%\setcounter{equation}{\value{mytempeqncnt}}
% IEEE uses as a separator
\hrulefill
% The spacer can be tweaked to stop underfull vboxes.
\vspace*{4pt}
\end{figure*}


\subsubsection{The battery remains full (${S_Q}\quad to\quad {S_Q}$ )}In this transition case, operation Mode I or II should be activated. Besides, the harvested energy during the operation can be any value since the battery is already full at the beginning of the transition. The transition probability is thus given by
%\setcounter{mytempeqncnt}{\value{equation}}
%\setcounter{equation}{43}
\begin{equation}
\begin{split}
{T_{Q,Q}}& =\left[1-{F_{\rm X}}\left( 2C \right)\right]+ \Pr \left\{ \kappa \left[{n}\right] =0 \right\} \left[{F_{\rm X}}\left( 2C  \right)\right].
\end{split}
\end{equation}

\subsubsection{The non-empty battery is discharged (${S_j}\quad to\quad {S_i}$ with $0 \le i <j \le Q$)}
Since the stored energy is reduced during the transition, Mode III should be invoked. Besides, the discharged amount of energy (i.e., $(j-i)$ levels of energy) should be equal to the required transmitted energy at the relay to guarantee that the residual energy after the discharge being $i$ levels. Thus the transition probability can be evaluated as follows
\begin{equation}
\begin{split}
{T_{j,i}} =&\Pr \bigg\{ \Upsilon \left[ n \right]  =  {\Upsilon _{\rm {III}}}, {E_R^{\rm X}} = \varepsilon_{j-i} \left| {{\Delta}[n]=0} \right. \bigg\}\\
 =&\Pr \left\{ \kappa \left[{n}\right] =1 \right\} \Pr \left\{ { {(j-i-1) C \over Q} < {{P_R^{\rm X}} \over 2} \le {(j-i) C \over Q } }\right\}  \\
 =& \Pr \left\{ \kappa \left[{n}\right] =1 \right\}\left[{F_{\rm X}}\left( 2(j-i)C \over Q \right)-\right.\\
&~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\left.{F_{\rm X}}\left( 2(j-i-1)C \over Q \right)\right] .
\end{split}
\end{equation}

We now define $\mathbf {Z}= ({T_{i,j}})$ to denote the $(Q+1) \times (Q+1)$ state transition matrix of relay battery. By using similar methods in \cite{Krikidis_CL_2012_RF}, we can readily verify that the transition matrix $\mathbf{Z}$ derived from the above MC model is irreducible and row stochastic. Hence, there must exist a unique stationary distribution $\pmb{\pi}$ that satisfies the following equation%T-matrix-satisfy}
\begin{equation}\label{eq:steady_state}
\pmb {\pi}  =\left( {{{\pi} _{0}},{{\pi} _{1}}, \cdots, {{\pi} _{Q}}} \right)^{T} = \left({\mathbf{Z}}\right)^{T} \pmb {\pi},
\end{equation}
where ${{\pi} _{i}}$, $i \in \left\{ {0,1, \cdots ,Q} \right\}
$, is the $i$-th component of $\pmb {\pi}$ representing the stationary distribution of the $i$-th energy level at relay. The battery stationary distribution can be solved based on (\ref{eq:steady_state}) and expressed as %[g5]%T-matrix-satisfy}
\begin{equation}\label{app-energy-distri}
 \pmb {\pi} = {\left( { {\mathbf{Z}}^{T} - \mathbf{I} + \mathbf{B} }\right)^{ - 1}}\mathbf{b},
\end{equation}
where ${\mathbf{B}_{i,j}}=1, \forall i, j$ and $\mathbf{b}={(1,1, \cdots ,1)^T}$.



